Manipulation Planning under Changing External Forces

In this work, we present a manipulation planning algorithm for a robot to keep an object stable under changing external forces. We particularly focus on the case where a human may be applying forceful operations, e.g. cutting or drilling, on an object that the robot is holding. The planner produces an efficient plan by intelligently deciding when the robot should change its grasp on the object as the human applies the forces. The planner also tries to choose subsequent grasps such that they will minimize the number of regrasps that will be required in the long-term. Furthermore, as it switches from one grasp to the other, the planner solves the problem of bimanual regrasp planning, where the object is not placed on a support surface, but instead it is held by a single gripper until the second gripper moves to a new position on the object. This requires the planner to also reason about the stability of the object under gravity.We provide an implementation on a bimanual robot and present experiments to show the performance of our planner.

==> Feasibilitycheck/Feasibilitycheck.tex <==
\section{Grasp Feasibility Check}
\label{sec:feasibility} 

We assume a system of $M$ manipulators, each with a gripper at the end. We
assume that the object has points on which a gripper can grip, e.g. the four
edges of the rectangular board.
In this work, we use the term \textit{grasp} to refer to the combined
placement of multiple grippers on the object.
Fig.~\ref{fig:sys} gives an example grasp using two grippers.
To place the grippers on these points on the object, the manipulators must
attain a certain joint configuration.  We use $q = {\left[ {{q^1}, \ldots
		,{q^M}} \right]^T}$ to refer to the joint angle configurations of $M$
manipulators, where $q^i$ is the configuration of the $i^{th}$ manipulator.  An
important concept in our formulation is the \textit{grasp configuration}, which
we use to refer to the joint angle configurations of the manipulators together
with the gripper placements on the object (the grasp). Note that, given an
object at a specified fixed pose, we can use the joint configuration $q$ and forward kinematics to find the gripper
placements on the object, i.e., the joint configuration $q$ by itself specifies a \textit{grasp configuration} with the implicit knowledge of 
the object pose.

Given an external force $f$ applied on the object, the question we try to
answer is: Will a given grasp configuration (i.e. the manipulators joints
\textit{and} the grasp) be able to keep the object stable?

%\subsection{Feasibility check based on grasp planning}
%
%--Figure
%The literature in grasp planning formulates it as an optimization problem. These methods usually begin with a geometrical model of the target object. Then
%they iteratively search for the optimal contact points on the grasped object based on grasp quality measures. In a general frictional case, denote the vector $\left( {f_1^c \ldots f_n^c} \right)$ of grasping forces at contact positions $p:\left\{ {{p_1}, \ldots ,{p_n}} \right\}$ as ${F^c}$, given an external wrench ${F^e}\in {\mathbb{R}^6}$ exerted on the object, grasp planning can be formulated as:
%
%\begin{equation}
%	\label{grasp}
%	\left\{ \begin{array}{l}
%		G{F^c} =  - {F^e}\\
%		{f_i^c} \in FC_i\\
%		0 \le \left\| {f_i^c} \right\| \le {F_i}\\
%		i = 1, \cdots ,n\\
%	\end{array} \right.
%\end{equation} 
%
%where $G$ is the grasp matrix and ${F_i}$ is the upper bound of ${f_i^c}$. In addition, ${f_i^c}$ is also constrained by its friction cone ${FC_i}$.
%
%Thus, checking whether the grasp positions $p$ is feasible to resist an external force can be regarded as checking whether there exists ${f_i^c}, i = 1, \cdots ,n$ that satisfies Eq.~\ref{grasp}. 
%
%These methods simply assume rigid contacts between robot fingers and objects, neglecting other physical properties of the robot and object system, such as object materials and robot finger stiffness. These properties will also influence the performance of grasp candidates, even they are feasible proved by Eq.~\ref{grasp}. For example, some robot hands are designedly covered with soft rubber, which will inevitably deform under external forces. Especially, grasp planning does not take the torque limitations of robot manipulator joints into account, which will also deteriorate the stability of the system under excessive external forces. In this case, grasp planning is not a good choice.

\subsection{Cooperative manipulation}
\begin{figure}[tp]
	\begin{center}
		\subfigure{{
				\includegraphics[width=3.2 in, angle=-0]{Feasibilitycheck/figs/system.pdf}}}

		\caption{A two-manipulator cooperative system holding a common object. }
		\label{fig:sys}
	\end{center}
	\vspace{-5mm}
\end{figure}


Suppose each manipulator is equipped with ${N^i}$ joints $\left( {i = 1, \ldots ,M} \right)$.  Fig. \ref{fig:sys} gives an example of the structure of a two-manipulator system. Denote the $\left( {6 \times 1} \right)$ vector of the generalized force acting at the ${i^{th}}$ gripper as ${f^{{g^i}}}$, the $\left( {{N^i} \times 1} \right)$ vector of torques at the joints of the ${i^{th}}$ manipulator as ${\tau ^i}$, the torque limits at the joints of the ${i^{th}}$ manipulator as $\tau _{\max }^i$, 
and the Jacobian of the ${i^{th}}$ manipulator at the configuration ${q^i}$ as ${J^i}$. 
Uchiyama et. al \cite{uchiyama1988symmetric,uchiyama1992symmetric} present the symmetric formulation for cooperative manipulation as: 

\begin{equation}
\label{eq:cooperative}
\begin{array}{l}
{J^T}{f^{\rm{g}}} =  \tau \\
W{f^g} =  - f\\
\left| \tau \right| \le {\tau _{\max }}
\end{array}
\end{equation} 

where ${J^T} = {\rm{Blockdiag}}(\mathop {{J^1}}\nolimits^T , \ldots ,\mathop {{J^M}}\nolimits^T )$, $\tau  = {[{\tau ^1}, \ldots ,{\tau ^M}]^T}$, ${\tau _{\max }} = {\left[ {\tau _{\max }^1, \ldots \tau _{\max }^M} \right]^T}$, ${f^g} = {[{f^{{g^1}}}, \ldots ,{f^{{g^M}}}]^T}$. $f$ is the vector of generalized external force applied on the object. $W$ (sometimes termed the grasp matrix \cite{mishra1987existence,ferrari1992planning,borst2004grasp}) is a $\left( {6 \times 6M} \right)$ matrix mapping the wrenches at the grippers to a resultant force on the object. 
%Note that a part of the each force at the grippers lies in the null space of $W$ and does not directly contribute to resisting external forces. These forces are usually termed the internal forces.


Eq.~\ref{eq:cooperative} mathematically describes the kinematic and static relationships between the generalized external force applied on the object and its counterparts required at the manipulator joints and grippers to resist it. It can be solved by linear programming, for example the Simplex method, to find a feasible solution of the forces and torques ${f^g}$ at the grip points and the corresponding torques $\tau$ at the manipulator joints to resist the external force.
Since $W$ usually has a non-trivial null space, there may be infinitely many solutions.

However, this formulation, lacking any constraints on the gripper forces ${f^g}$, assumes 
%rigid grasps among manipulators and the object and 
that the object is tightly attached to each gripper and that
%. That is, it assumes that 
the grippers can apply arbitrary wrenches on the object. 
In our task, the operation can also fail due to the load on the grip points.
%As discussed in Section \ref{sec:intro}, a cooperative manipulation may fail because of many physical and mechanical constraints, such as limited squeeze force of robot hands, flexible fingertips and material deformation. 
To solve this problem, we propose to model each grip with \textit{virtual joints}, with their own force/torque limits.

\subsection{Virtual joints}
\input{Feasibilitycheck/virtual_joints.tex}

%\begin{figure*}[tp]
%	\begin{center}
%		\mbox{
%			
%			\subfigure[Grasp Space]{{
%					\label{subfig:paths}
%					\includegraphics[width=2.75 in, angle=-0]{Feasibilitycheck/figs/paths.pdf}}}
%			
%			\subfigure[Sampling]{{
%					\label{subfig:samples}
%					\includegraphics[width=1.6 in, angle=-0]{Feasibilitycheck/figs/sample.pdf}}}	
%			
%			\subfigure[Manipulation path]{{
%					\label{subfig:graph}
%					\includegraphics[width=1.9 in, angle=-0]{Feasibilitycheck/figs/graph.pdf}}}		
%			
%		}	
%		\caption{Manipulation planning in the grasp space. Each sample within the grasp space in (b) represent a bimanual grasp. Each sample on the axes represents a single gripper grasp. For example, samples on the horizontal axis represent grasps of only gripper 1. }
%		\label{fig:graspspace}
%	\end{center}
%\end{figure*}


\begin{figure*}[tbp]
	\begin{center}
		\mbox{
			
			\subfigure[Grasp Space]{{
					\label{subfig:paths}
					\includegraphics[width=2.75 in, angle=-0]{Manipulation/figs/paths.pdf}}}
			
			\subfigure[Sampling]{{
					\label{subfig:samples}
					\includegraphics[width=1.6 in, angle=-0]{Manipulation/figs/sample.pdf}}}	
			
			\subfigure[Manipulation path]{{
					\label{subfig:graph}
					\includegraphics[width=2.0 in, angle=-0]{Manipulation/figs/graph.pdf}}}		
			
		}	
		\caption{Manipulation planning in the grasp space. }
		\label{fig:graspspace}
	\end{center}
	\vspace{-5mm}
\end{figure*}


As shown in Fig. \ref{fig:subfig:six}, we propose to represent each grip with three prismatic joints and three revolute joints along orthogonal directions $xyz$. We assume that the prismatic joints have limits on the forces they can apply along the $xyz$ directions denoted as $P_x$, $P_y$ and $P_z$, while the revolute joints have limits on the torques as $R_x$, $R_y$ and $R_z$ respectively.


We use the maximum external force  a prismatic joint can resist to represent the grip's capacity to avoid potential liner motions along its joint axis, and we use the maximum external torque a revolute joint can resist to represent the grip's capacity to avoid potential rotational motions about its joint axis. Therefore the force/torque limits of these virtual joints represent the forces/torques at which the grip starts to fail. For example, suppose we apply a downward force $f$ on the top of the object as shown in Fig.~\ref{fig:subfig:prismatic}. We start from a small force.  As we increase the force, the object may start to slide between the fingers at some point. This gives us the limit, $P_x$, of the prismatic joint along $x$. Therefore we can find the value of $P_x$ by increasing the magnitude of the force along that direction and identifying the value that makes the object start to slide. Similarly, as shown in Fig.~\ref{fig:subfig:revolute}, we can apply a torque (a force $f$ at a distance $d$) about the axis $y$. As we increase the torque at some point, the object will deviate from its desired pose more than an acceptable threshold. Therefore, we can increase the torque, in practice either $f$ or $d$, gradually to find the torque value which gives us the torque limit ${R_y}$. We propose to find the limits ($P_x$, $P_y$, $P_z$)  of all prismatic joints and the limits ($R_x$, $R_y$, $R_z$) of all revolute joints for a gripper and a given object similarly.
These values depend on the material of the object, and therefore the robot needs a calibration step when an object with a new material is used.
%We can then use these limits to check whether a feasible set of forces and torques exists at the grip points.

\subsection{Grasp feasibility check using virtual joints}

We introduce a $\left( {6 \times 1} \right)$ vector $f_{\max }^i = \left[ {{P_x},P{}_y,{P_z},{R_x},{R_y},{R_z}} \right]$ to represent the limits of ${i^{th}}$ gripper's virtual joints. 
%As discussed above, it describes the maximum forces and torques the ${i^{th}}$ gripper's can apply on the object. 
Thus, we can modify Eq. \ref{eq:cooperative} as:

\begin{equation}
\label{eq:virtual_cons}
\begin{array}{l}
{J^T}{f^{\rm{g}}} =  \tau \\
W{f^g} =  - f\\
\left| \tau \right| \le {\tau _{\max }}\\
\left| {{f^g}} \right| \le {f_{{{\max }^{}}}}
\end{array}
\end{equation} 

where ${f_{\max }} = {\left[ {f_{\max }^1, \ldots ,f_{\max }^M} \right]^T}$. 

%Using Eq. \ref{eq:virtual_cons}, we can check whether a certain grasp configuration fails in terms of breaking the limits of the virtual joints on the grip points or the real joints of the manipulators. 
Thus, given an external force $f$, using Eq. \ref{eq:virtual_cons} we can identify the feasibility of a candidate grasp configuration $q$ by checking whether a feasible $f^g$ and $\tau$ for Eq. \ref{eq:virtual_cons} exist.
%Eq. \ref{eq:virtual_cons}  gives a tool to figure out how much torque and force the cooperative manipulators should apply at their joints and grippers to resist an external force. 
Eq. \ref{eq:virtual_cons} can again be solved by linear programming.  
%Note that when we find a feasible solution to Eq. \ref{eq:virtual_cons}, we are checking that there is at least one solution. We assume that the underlying controllers will be able to realize that solution.
In Sec. \ref{subsec:verification},  we show how we measure virtual joint limits and we present experiments on a real robot to demonstrate how these limits perform in real applications.






==> Feasibilitycheck/virtual_joints.tex <==
\begin{figure}[tp]
	\begin{center}

		\mbox{
			
			
			\subfigure[Virtual joints]{{
					\label{fig:subfig:six}  
					\includegraphics[width=1.07 in, angle=-0]{Feasibilitycheck/figs/virtualjoint.pdf}}}
			
			\subfigure[Prismatic along $x$ ]{{
					\label{fig:subfig:prismatic}  
					\includegraphics[width=1.07 in, angle=-0]{Feasibilitycheck/figs/rotational.pdf}}}
			
			\subfigure[Revolute about $y$]{{
					\label{fig:subfig:revolute}  
					\includegraphics[width=1.04 in, angle=-0]{Feasibilitycheck/figs/prismatic.pdf}}}
			
		}
		\caption{We use three prismatic joints and three revolute joints to represent each grasp. Two of them are shown in (b) and (c). }
		\label{fig:virtuals}
	\end{center}
	\vspace{-5mm}
\end{figure}


==> Implementation/integratedplanning/integratedplanning.tex <==
\subsection{Real experiments}
\label{subsec:realexperiments}
In this section, ...

We present complete executions of plans on the real robot in the attached video. At the end
of the video, we also present a common failure case, which is due to the gripper
fingers hitting the object during re-grasping motion.

==> Implementation/planning_cutting/planning_cutting.tex <==
\subsubsection{Planning for tasks that involve cutting}
\label{subsec:planningwithcutting}
After our initial set of experiments, we noticed that the limits of virtual joints shown in Table \ref{table:measurement} are not large enough to resist the forces if we want to cut the object as in Fig.~\ref{fig:cutting:f}. We measured that the external force of such a cutting operation varies between $30N$ to $60N$. The failure is essentially due to the limited frictional forces between the object and the robot fingers. However, if the robot grasps the object with the object resting on the palms of the grippers as shown in Fig.~\ref{fig:cutting:f}, the virtual joint limits along the corresponding axes would be much higher, since the virtual joint limits would basically depend on the stiffness of the gripper palms. Therefore, with this setup, we created a new task with four drilling operations and one cutting operation as shown in Fig. \ref{fig:cutting}. We modified the virtual joint limit $P_x$ to be $\infty $ and implemented the min-regrasp planner on the task. It was able to find a stable solution as presented in Fig.~\ref{fig:cutting}.
The robot can still \textbf{not} resist the cutting force by the grasp configurations shown in Fig.~\ref{fig:cutting:b}-\ref{fig:cutting:e}. Therefore the planner chooses to the grasp configuration as shown in Fig.~\ref{fig:cutting:f} to resist the cutting force. The planner needs only two regrasps.


%\input{Implementation/real_experiments/figs/fig_drilling.tex}
\vspace{5mm}

==> Implementation/planning_cutting/tables/table_cutting.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
	\centering
	\caption{Resulting of three planners on 100 cutting tasks. Each task involves 4 drilling operations at the surface of a foam board and one cutting operation from the top of the board}
	\label{table:A4-cutting}
	\begin{center}
	\begin{tabular}{@{}cccccc@{}}
		\toprule
		\multirow{2}{*}{Planner} & \multicolumn{2}{c}{Regrasps} &  & \multicolumn{2}{c}{Planning Time} \\ \cmidrule(lr){2-3} \cmidrule(l){5-6} 
		& mean          & std          &  & mean            & std             \\ \midrule
		Random              & 9.99          & 0.11         &  & 7.14            & 1.53            \\
		Greedy                   & 4.66          & 0.52         &  & 2.62            & 0.27            \\
		Min-regrasp              & 2             & 0            &  & 2.97            & 0.23            \\ \bottomrule
	\end{tabular}
	\end{center}
\end{table}

==> Implementation/planning_drilling/figs/fig_sin.tex <==
\begin{figure*}[tbhp]
	\begin{center}
		
		\mbox{
			
			
			\subfigure{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1.3 in, angle=-0]{Implementation/planning_drilling/figs/sin5/sin-1.jpg}}}
			
			\subfigure{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1.3 in, angle=-0]{Implementation/planning_drilling/figs/sin5/sin-2.jpg}}}
			
			\subfigure{{
					\label{fig:subfig:A4-ran-force-1}  
					\includegraphics[width=1.3 in, angle=-0]{Implementation/planning_drilling/figs/sin5/sin-3.jpg}}}
			
			\subfigure{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1.3 in, angle=-0]{Implementation/planning_drilling/figs/sin5/sin-4.jpg}}}
			
			\subfigure{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1.3 in, angle=-0]{Implementation/planning_drilling/figs/sin5/sin-5.jpg}}}

			
		}

		
		
			
		\caption{A plan generated by the min-regrasp planner for a sine-drilling task.}
		\label{fig:sin-drilling}
	\end{center}
\end{figure*}

==> Implementation/planning_drilling/figs/fig_tick_min.tex <==
\begin{figure}[tbhp]
	\begin{center}

		
		\mbox{
			
			
			\subfigure{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=0.94 in, angle=-0]{Implementation/planning_drilling/figs/tick2/tick-1.jpg}}}
	%		\hspace{1 in}
			\subfigure{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1.125 in, angle=-0]{Implementation/planning_drilling/figs/tick2/tick-m.jpg}}}	
	
	
			\subfigure{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=0.94 in, angle=-0]{Implementation/planning_drilling/figs/tick2/tick-2.jpg}}}

			
		}
		
			
		\caption{A plan generated by the min-regrasp planner for a tick-drilling task.}
		\label{fig:tick-min}
	\end{center}
\end{figure}




==> Implementation/planning_drilling/planning_drilling.tex <==
\subsection{Performance of multi-step manipulation planning}
\label{subsec:planningwithdrilling}

%\input{Implementation/planning_drilling/tables/table_drilling_ran.tex}
\input{Implementation/planning_drilling/tables/numberOfregrasp.tex}
\input{Implementation/planning_drilling/tables/time.tex}
\input{Implementation/planning_drilling/figs/fig_ran.tex}
\input{Implementation/planning_drilling/figs/fig_tick_greedy.tex}

In this section, we tested the performance of the multi-step manipulation planners proposed in Sec.~\ref{sec:manipulation}  in terms of minimizing the number of regrasps and planning efficiency.


\subsubsection{Planning for drilling}

First, we tested our planners on three types of tasks, including:
\begin{itemize}
	\item \textit{random-drilling:} Each example contains 10 drilling points randomly distributed on the surface of the board. An example is shown in Fig.~\ref{fig:drilling-ran};
	\item \textit{tick-drilling}: Each example contains 40 drilling forces along two random line segments meeting at a common point. Three examples are shown in Table~\ref{table:ran};
	\item \textit{sine-drilling}: Each example contains 40 drilling forces along the sinusoidal curve shown in Table~\ref{table:ran}.
\end{itemize}

For all the drilling tasks, we randomly changed the magnitude of the drilling force to be between $10 N$ to $15 N$ and we assume the forces are normal to the surface of the board. 

We introduce a \textit{random planner} as a baseline approach. For the first
external force, the random planner samples a random grasp in the grasp space
until it finds a feasible one. For any subsequent force, it first checks
whether the feasible grasp for the preceding force is still feasible. If not,
it falls back to random sampling. 



We compared the performance of our planners, min-regrasp and greedy, with the
random planner in terms of the number of regrasps and planning time. All three
planners were implemented in OpenRAVE simulation environment and as the motion
planner to connect two configurations, we used the BiRRT planner
\cite{kuffner2000rrt} as implemented in OpenRAVE.


%\input{Implementation/planning_drilling/figs/fig_tick_min.tex}
%\input{Implementation/planning_drilling/figs/fig_sin.tex}

We generated 100 random examples for each type of the tasks above.
Table~\ref{table:ran} shows the average results of the three planners on the 100 random instances of each type of task. For the random-drilling tasks, the random planner generates almost one bimanual regrasp for every external force (maximum 18 regrasps for 10 external forces). The min-regrasp does dramatically minimize the number of regrasps (5 regrasps for 10 external forces, an example solution is shown in Fig.~\ref{fig:drilling-ran}) and cut down the planning time.
The greedy planner also performs well in terms of reducing regrasps (8 regrasps) and planning time.

\input{Implementation/real_experiments/figs/fig_drilling.tex}
Similarly, the random planner generates plans with a large number of regrasps (49 regrasps for 40 external forces of each tick-drilling task and 76 regrasps for 40 external forces of each sine-drilling task), while min-regrasp planner just needs 1.3 regrasps for the tick-drilling tasks (an example solution is shown in Fig.~\ref{fig:real-tick}) and 4 regrasps for the sine-drilling tasks on average. The greedy planner shows a much better performance compared with the random planner, but worse than the min-regrasp planner. For example, as shown in Fig.~\ref{fig:tick-greedy}, the greedy planner requires the grippers to climb along the edges of the board up and down frequently to follow the movements of the external forces, while the min-regrasp planner comes up with a plan of just two regrasps in Fig.~\ref{fig:real-tick}. We present a complete run of such a plan on the real robot in the attached video.

We also counted the number of samples the random planner needed before it found
a feasible grasp.  On average, the random planner needed 35.8 samples for each
external force, showing that planning is necessary and random grasps have
little chance of being feasible.

%\emph{Note that, the experiments show that the random planner needs 38.2 trials for each external force in the random-drilling tasks, 22.4 trials for each force in the tick-drilling tasks and 48.6 trials for each force in the sine-drilling tasks. Therefore, it is difficult to find a feasible grasp in the grasp space to resist an external force. }

Note that most of the planning time shown in Table~\ref{table:ran} is spent by
the motion planner (BiRRT). The role of the graph search (e.g. greedy vs.
min-regrasp), however, is crucial in reducing the planning time, since the
number of required BiRRT runs is determined by the number of regrasps, which in
turn is determined by the graph search algorithm. 

Our planners are not limited to grasping rectangular objects. To demonstrate
this, we tested the min-regrasp planner on a circular board with a sequence of
40 circular drilling operations. A plan of only two regrasps is in Fig.~\ref{fig:circular}.

\input{Implementation/planning_drilling/figs/fig_circle.tex}


==> Implementation/planning_drilling/tables/numberOfregrasp.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
	\centering
	\caption{Results of three planners on three different drilling\&cutting tasks.}
	\label{table:regrasp}
	\begin{tabular}{@{}cccc@{}}
		\toprule
		& Random-drilling & Tick-drilling & Drilling\&cutting \\ \midrule
		Random      & 17.6(0.9)       & 48.7(10.7)    & 75.8(1.7)         \\
		Greedy      & 7.8(1.9)        & 4.3(2.4)      & 7.0(0.8)          \\
		Min-regrasp & 5.2(0.9)        & 1.3(1.0)      & 4.4(0.5)          \\ \bottomrule
	\end{tabular}
\end{table}

==> Implementation/planning_drilling/tables/table_drilling_ran.tex <==



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
%\begin{table*}[tb]
%	\centering
%	\caption{Results of three planners on 100 drilling tasks. Each task involves a certain number of drilling operations distributed on the surface of foam boards. Times are in seconds}
%	\label{table:ran}
%	\begin{tabular}{@{}ccclcclcc@{}}
%		\toprule
%		& \multicolumn{2}{c}{random-drilling} &  & \multicolumn{2}{c}{sine-drilling} &  & \multicolumn{2}{c}{tick-drilling} \\ \cmidrule(lr){2-3} \cmidrule(lr){5-6} \cmidrule(l){8-9} 
%		& \# of regrasp      & Planning time      &  & \# of regrasp     & Planning time     &  & \# of regrasp     & Planning time     \\ \cmidrule(r){1-3} \cmidrule(lr){5-6} \cmidrule(l){8-9} 
%		Random      & 17.6(0.9)      & 174.2(4.7)         &  & 75.8(1.7)     & 758.6(21.7)       &  & 48.7(10.7)     & 437.8(31.3)        \\
%		Greedy      & 7.8(1.9)       & 65.3(16.1)         &  & 7.0(0.8)      & 78.9(8.1)         &  & 4.3(2.37)      & 51.95(5.78)        \\
%		Min-regrasp &\textbf{ 5.2(0.9)}       & \textbf{45.7(6.6) }         &  & \textbf{4.4(0.5)}      & \textbf{56.2(5.0)}         &  &\textbf{ 1.31(1.04) }     & \textbf{45.1(3.8)}       \\ \bottomrule
%	\end{tabular}
%\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
%\begin{table*}[]
%	\centering
%	\caption{Results of three planners on 100 drilling tasks. Each task involves a certain number of drilling operations distributed on the surface of foam boards. Times are in seconds}
%	\label{table:ran}
%	\begin{tabular}{@{}cccccccccc@{}}
%		\toprule
%		\multirow{2}{*}{} & \multicolumn{2}{c}{random-drilling} &  & \multicolumn{2}{c}{sine-drilling} &  & \multicolumn{2}{c}{tick-drilling} & \multirow{5}{*}{	\includegraphics[width=1.05 in, angle=-0]{Implementation/planning_drilling/tables/curves}} \\ \cmidrule(lr){2-3} \cmidrule(lr){5-6} \cmidrule(lr){8-9}
%		& \# of regrasp    & planning time    &  & \# of regrasp   & planning time   &  & \#of regrasp    & planning time   &                   \\ \cmidrule(r){1-3} \cmidrule(lr){5-6} \cmidrule(lr){8-9}
%		Random        & 17.6(0.9)      & 174.2(4.7)         &  & 75.8(1.7)     & 758.6(21.7)       &  & 48.7(10.7)     & 437.8(31.3)              &                   \\
%		Greedy           & 7.8(1.9)       & 65.3(16.1)         &  & 7.0(0.8)      & 78.9(8.1)         &  & 4.3(2.4)      & 52.0(5.8)              &                   \\
%		Min-regrasp        &\textbf{ 5.2(0.9)}       & \textbf{45.7(6.6) }         &  & \textbf{4.4(0.5)}      & \textbf{56.2(5.0)}         &  &\textbf{ 1.3(1.0) }     & \textbf{45.1(3.8)}              &                   \\ \bottomrule
%	\end{tabular}
%\end{table*}




% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[tp]
	\centering
	\caption{Results of three planners on three drilling tasks. 
		%Each task involves a certain number of drilling operations distributed on the surface of foam boards. 
		Times are in seconds. Std deviations are in parantheses.}
	\label{table:ran}
	\begin{tabular}{@{}cccccccccc@{}}
		\cmidrule(r){1-9}
		\multirow{2}{*}{} & \multicolumn{2}{c}{random-drilling} &  & \multicolumn{2}{c}{tick-drilling} &  & \multicolumn{2}{c}{sine-drilling} & \multirow{5}{*}{	\includegraphics[width=1.08 in, angle=-0]{Implementation/planning_drilling/tables/curves}} \\ \cmidrule(lr){2-3} \cmidrule(lr){5-6} \cmidrule(lr){8-9}
		& \# of regrasp    & planning time    &  & \# of regrasp   & planning time   &  & \#of regrasp    & planning time   &                    \\ \cmidrule(r){1-3} \cmidrule(lr){5-6} \cmidrule(lr){8-9}
		Random      & 17.6(0.9)      & 174.2(4.7)                &  & 48.7(10.7)     & 437.8(31.3)     &  & 75.8(1.7)     & 758.6(21.7)            &                    \\
		Greedy         & 7.8(1.9)       & 65.3(16.1)                  &  & 4.3(2.4)      & 52.0(5.8)      &  & 7.0(0.8)      & 78.9(8.1)         &                    \\
		Min-regrasp      &\textbf{ 5.2(0.9)}       & \textbf{45.7(6.6) }                  &  &\textbf{ 1.3(1.0) }     & \textbf{45.1(3.8)} &  & \textbf{4.4(0.5)}      & \textbf{56.2(5.0)}           &                    \\ \cmidrule(r){1-9}
	\end{tabular}
\end{table*}

==> Implementation/planning_drilling/tables/table_drilling_sin.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
	\centering
	\caption{Resulting of three planners on 100 drilling tasks. Each task involves 40 drilling operations uniformly distributed along a sin curve on a foam board.}
	\label{table:A3-sin}
	\begin{center}
	\begin{tabular}{@{}cccccc@{}}
		\toprule
		\multirow{2}{*}{Planner} & \multicolumn{2}{c}{Regrasps} &  & \multicolumn{2}{c}{Planning Time} \\ \cmidrule(lr){2-3} \cmidrule(l){5-6} 
		& Mean          & Std          &  & Mean            & Std             \\ \midrule
		One-by-one               & 77.43         & 0.87         &  & 44.00           & 14.10           \\
		Greedy                   & 7.01          & 0.80         &  & 18.88           & 0.98            \\
		Min-regrasp              & 4.40          & 0.53         &  & 19.01           & 0.65            \\ \bottomrule
	\end{tabular}
	\end{center}
\end{table}

==> Implementation/planning_drilling/tables/table_drilling_tick.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
	\centering
	\caption{Resulting of three planners on 100 drilling tasks. Each task involves 40 drilling operations uniformly distributed along a tick curve on a foam board.}
	\label{table:A3-tick}
	\begin{center}
	\begin{tabular}{@{}cccccc@{}}
		\toprule
		\multirow{2}{*}{Planner} & \multicolumn{2}{c}{Regrasps} &  & \multicolumn{2}{c}{Planning Time} \\ \cmidrule(lr){2-3} \cmidrule(l){5-6} 
		& Mean          & Std          &  & Mean             & Std            \\ \midrule
		One-by-one               & 79.40         & 0.74         &  & 48.78            & 3.09           \\
		Greedy                   & 6.01          & 2.13         &  & 7.86             & 0.63           \\
		Min-regrasp              & 2             & 0            &  & 7.92             & 0.54           \\ \bottomrule
	\end{tabular}
\end{center}
\end{table}

==> Implementation/planning_drilling/tables/time.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
	\centering
	\caption{Planning time for both heavy and light objects. Times are in seconds. Standdeviations are in parantheses. The planner is set to generate a set of 20 feasible samples for each intersection.}
	\label{table-time}
	\begin{tabular}{@{}ccccccccccccccc@{}}
		\toprule
		\multirow{2}{*}{} & \multicolumn{4}{c}{random-drilling} &  & \multicolumn{4}{c}{tick-drilling} &  & \multicolumn{4}{c}{drilling\&cutting} \\ \cmidrule(lr){2-5} \cmidrule(lr){7-10} \cmidrule(l){12-15} 
		& l1  & l2  & l3        & l4          &  & l1 & l2 & l3        & l4          &  & l1  & l2  & l3         & l4           \\ \cmidrule(r){1-5} \cmidrule(lr){7-10} \cmidrule(l){12-15} 
Heavy             & 11.6(2.8)   & 0.0(0.0)   & 50.1(4.7) & 440.0(62.3) &  & 12.9(1.0)  & 0.0(0.0)  & 12.8(1.0) & 114.4(17.3) &  & 2.79(0.2)   & 0.0(0.0)   & 20.6(1.2)  & 139.1(25.0)  \\
Light             & 11.6(2.8)   & 0.0(0.0)   & 17.8(1.9) & 155.5(11.4) &  & 12.9(1.0)   & 0.0(0.0)  & 5.0(0.3)  & 39.8(8.3)   &  & 2.79(0.2)    & 0.0(0.0)   & 6.6(0.7)   & 71(14.1)     \\ \bottomrule
	\end{tabular}
\end{table*}

==> Implementation/real_experiments/figs/fig_circle.tex <==
\begin{figure}[htpb]
	\begin{center}
		\mbox{


			\subfigure[]{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1. in, angle=-0]{Implementation/planning_drilling/figs/circle/round-1.png}}}

			\subfigure[]{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1. in, angle=-0]{Implementation/planning_drilling/figs/circle/round-2.png}}}
			\subfigure[]{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1. in, angle=-0]{Implementation/planning_drilling/figs/circle/round-3.png}}}
			
		}
		


	
		\caption{Solutions generated by min-regrasp planner for a drilling task on a foam board. }
		\label{fig:tick}
	\end{center}
\end{figure}

==> Implementation/real_experiments/figs/fig_tick.tex <==
\begin{figure*}[htpb]
	\begin{center}
		\mbox{


			\subfigure[]{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1. in, angle=-0]{Implementation/planning_drilling/figs/tick12/tickr-1.png}}}

			\subfigure[]{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1. in, angle=-0]{Implementation/planning_drilling/figs/tick12/tickr-2.png}}}
			\subfigure[]{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1. in, angle=-0]{Implementation/planning_drilling/figs/tick12/tickr-3.png}}}
		
			\subfigure[]{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1. in, angle=-0]{Implementation/planning_drilling/figs/tick12/tickr-4.png}}}

			\subfigure[]{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1. in, angle=-0]{Implementation/planning_drilling/figs/tick12/tickr-5.png}}}

			\subfigure[]{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1. in, angle=-0]{Implementation/planning_drilling/figs/tick12/tickr-6.png}}}
			
		}
		

		\mbox{
			
			
			\subfigure[]{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1. in, angle=-0]{Implementation/planning_drilling/figs/tick12/tickr-7.png}}}
			
			\subfigure[]{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1. in, angle=-0]{Implementation/planning_drilling/figs/tick12/tickr-8.png}}}
			\subfigure[]{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1. in, angle=-0]{Implementation/planning_drilling/figs/tick12/tickr-9.png}}}
			
			\subfigure[]{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1. in, angle=-0]{Implementation/planning_drilling/figs/tick12/tickr-10.png}}}
			
			\subfigure[]{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1. in, angle=-0]{Implementation/planning_drilling/figs/tick12/tickr-11.png}}}
			
			\subfigure[]{{
					\label{fig:subfig:measure_c}  
					\includegraphics[width=1. in, angle=-0]{Implementation/planning_drilling/figs/tick12/tickr-12.png}}}
			
		}
		
	
		\caption{Solution for a tick-drilling task generated by greedy planner. The solution involves 11 regrasps which switch along the tick line. }
		\label{fig:tick}
	\end{center}
\end{figure*}

==> Implementation/real_experiments/real_experiments.tex <==
\subsection{Real robot execution}
\label{subsec:planningwithdrilling}

We executed plans generated by our planner on a Baxter robot and performed
drilling and cutting operations. 

During these executions, there were frequent failures, all due to 
motions of the robot arm during re-grasping. When re-grasping, as the robot
approaches the board with its gripper,
there is small clearance between the two fingers of the gripper and the width
of the board. Therefore, small uncertainties in the position of the board meant
that a finger can hit the board and cause the plan to fail. We show an example
failure case at the end of the attached video. 
These failures due to uncertainty in the object pose were not unexpected: the
motion planner we use to perform the re-grasp actions do not take into account
object pose uncertainty. These problems can be 

When re-grasp motions were completed without problems, the robot was
able to execute the plans, it kept
the object stable against all the drilling and cutting
forces, and the tasks were completed successfully. 
We present snapshots from two such successful plans in Fig.~\ref{fig:cutting} and Fig. \ref{fig:real-tick}.
Please see the attached video for complete runs. 

%\input{Implementation/real_experiments/figs/fig_drilling.tex}


==> Implementation/regrasp/figs/fig_h.tex <==
\begin{figure*}[tbp]
	\begin{center}
		\mbox{


			\subfigure{{
					\label{fig:subfig:h1}  
					\includegraphics[width=1.3 in, angle=-0]{Implementation/regrasp/figs/h-1}}}

			\subfigure{{
					\label{fig:subfig:h2}  
					\includegraphics[width=1.3 in, angle=-0]{Implementation/regrasp/figs/h-2}}}

			\subfigure{{
					\label{fig:subfig:h3}  
					\includegraphics[width=1.3 in, angle=-0]{Implementation/regrasp/figs/h-3}}}
			
			\subfigure{{
					\label{fig:subfig:h4}  
					\includegraphics[width=1.3 in, angle=-0]{Implementation/regrasp/figs/h-4}}}
			
			\subfigure{{
					\label{fig:subfig:h5}  
					\includegraphics[width=1.3 in, angle=-0]{Implementation/regrasp/figs/h-5}}}							
		}
	
		\caption{Regrasping a heavy object.}
		\label{fig:h}
	\end{center}
\end{figure*}

==> Implementation/regrasp/figs/fig_light.tex <==
\begin{figure*}[tbp]
	\begin{center}
		\mbox{


			\subfigure[Start configuration]{{
					\label{fig:subfig:light-start}  
					\includegraphics[width=1.35 in, angle=-0]{Implementation/regrasp/figs/light-1}}}

			\subfigure[Release]{{
					\label{fig:subfig:light1}  
					\includegraphics[width=1.35 in, angle=-0]{Implementation/regrasp/figs/light-2}}}

			\subfigure[Regrasp]{{
					\label{fig:subfig:light2}  
					\includegraphics[width=1.35 in, angle=-0]{Implementation/regrasp/figs/light-3}}}
			
			\subfigure[Release]{{
					\label{fig:subfig:light3}  
					\includegraphics[width=1.35 in, angle=-0]{Implementation/regrasp/figs/light-4}}}
			
			\subfigure[Regrasp/Target Config.]{{
					\label{fig:subfig:light-target}  
					\includegraphics[width=1.35 in, angle=-0]{Implementation/regrasp/figs/light-5}}}							
		}

		
		\caption{Regrasping a light object.}
		\label{fig:light}
	\end{center}
\end{figure*}

==> Implementation/regrasp/regrasp.tex <==
\subsection{Performance of regrasp planner}
\label{subsec:planningwithdrilling}

\input{Implementation/regrasp/figs/fig_light.tex}
\input{Implementation/regrasp/figs/fig_m.tex}
\input{Implementation/regrasp/figs/fig_h.tex}


We tested the performance of the regrasp planner proposed in Sec.~\ref{sec:regrasp} on \textit{light}, \textit{medium} and \textit{heavy} objects respectively. For each problem, the planner takes the start $q_s$ and target configuration $q_t$ as inputs. Then, it outputs motion trajectories $T$ for the robot to regrasp the object.

For the \textit{light }object, the robot is expected to change its grasp on the object from Fig.~\ref{fig:subfig:light-start} to Fig.~\ref{fig:subfig:light-target}. 
Since the object is light relative to the capability of manipulators, the robot can stably grasp and move it using just one single hand at most reachable configurations. In this scenario, Fig~\ref{fig:light} shows one solution for the problem. As the figure shows, the robot directly releases off and regrasps the object, without the need of reorienting it to intermediate configurations. 

For the \textit{medium }heavy object, as discussed in Sec.~\ref{sec:regrasp}, the object may slip down between gripper fingers if the robot directly release one hand. That is, the robot probably needs to move to some intermediate configurations at which one single hand can keep the object stable. 
Fig.~\ref{fig:m} shows a solution to regrasp a medium heavy object. The robot transfers the object to configurations in Fig.~\ref{fig:subfig:m-start} and \ref{fig:subfig:m2} before releasing one hand. After releasing, most object weight will be resisted by the force bending gripper fingers as shown in Fig.~\ref{fig:subfig:m1} and \ref{fig:subfig:m3}, which is much larger than the frictional force between the object and finger surfaces.

Fig.~\ref{fig:h} gives one solution to regrasp a\textit{ heavy} object from the $g_{s}$ and $g_{t}$ in Fig.~\ref{subfig:prob}.  In such a scenario, the robot may use its palms (which could offer far larger support force compared with gripper fingers and will also be used to resist large external forces in Sec.~\ref{subsec:planningwithdrilling}) to counterbalance the object weight, since it is too heavy for the robot grippers. As Fig. \ref{fig:h} shows, the robot releases and regrasps the object at two configurations where one robot palm is used to resist its weight respectively.

Table shows the average planning time of 100 runs for each problem. As the table show, most time is spent on dual-arm motion planing, while the time for sampling feasible intermediate configurations is negligible.

\textbf{Table here}


==> Manipulation/Manipulation.tex <==
\section{Multi-step manipulation planning}
\label{sec:manipulation} 

%\begin{figure*}[tp]
%	\begin{center}
%		\mbox{
%			
%			\subfigure[Grasp Space]{{
%					\label{subfig:paths}
%					\includegraphics[width=2.75 in, angle=-0]{Manipulation/figs/paths.pdf}}}
%			
%			\subfigure[Sampling]{{
%					\label{subfig:samples}
%					\includegraphics[width=1.6 in, angle=-0]{Manipulation/figs/sample.pdf}}}	
%			
%			\subfigure[Manipulation path]{{
%					\label{subfig:graph}
%					\includegraphics[width=2.0 in, angle=-0]{Manipulation/figs/graph.pdf}}}		
%			
%		}	
%		\caption{Manipulation planning in the grasp space. }
%		\label{fig:graspspace}
%	\end{center}
%\end{figure*}

Our goal is to automatically generate a sequence of robot grasp configurations ${Q:\left\{ {{q_1}, \ldots ,{q_N}} \right\}}$ and robot trajectories ${T:\left\{ {{t_1}, \ldots ,{t_N}} \right\}}$ to hold an object $O$ stable against a sequence of external forces $F:\left\{ {{f_1}, \ldots ,{f_N}} \right\}$, where ${t_i}$ represents the manipulators' trajectories to move from ${q_{i-1}}$
 to ${q_i}$. 
The problem is to generate an efficient manipulation plan that minimizes the number of regrasps. To do this, we first define the \textit{grasp space}.
%, which is similar to the contact space in Lee et. al \cite{lee2015hierarchical}.

\begin{figure*}[tbp]
	\begin{center}
		\mbox{
			
			\subfigure[Grasp Space]{{
					\label{subfig:paths}
					\includegraphics[width=2.75 in, angle=-0]{Manipulation/figs/manipulation.pdf}}}
			\subfigure[Manipulation path]{{
					\label{subfig:graph}
					\includegraphics[width=2.0 in, angle=-0]{Manipulation/figs/graph.pdf}}}		
			
		}	
		\caption{Manipulation planning in the grasp space. }
		\label{fig:graspspace}
	\end{center}
	\vspace{-5mm}
\end{figure*}


\subsection{Grasp space}

%Still, take the system of the Baxter robot and a rectangular board in Fig. \ref{subfig:manupulator} for example. In the system, the robot is supposed to hold the object using bimanual grasps on the edges of the board.  Based on the number of manipulators and the grasp area of the target object, we can build a grasp space such that each point in the space corresponds to a grasp of the object. Fig. \ref{subfig:graspspace} shows the two-dimensional grasp space for the system in Fig. \ref{subfig:manupulator}. In the grasp space, the $x$ axis corresponds to the grip position of the left hand on the board edges, while the $y$ axis corresponds to the grip position of right hand. For example, the point ${G_1}$ in the grasp space determines the Baxter's grip positions in \ref{subfig:manupulator}.

%We assume each manipulator to have a gripper as the end-effector. 
We assume we know a set of points on the object on which a gripper can be placed. For example, in Fig.~\ref{subfig:paths}, a gripper of the Baxter robot can grip any point on the edges of the board (between corners ${A - B - C - D}$). We define a \textit{grasp space} as shown in Fig.~\ref{subfig:paths}, such that the axes are the possible gripper positions, and each point in the space specifies a grasp. For example, the point $G1$ determines Baxter's grasp in Fig. \ref{subfig:paths}-top, while the point $G5$ specifies the grasp in Fig. \ref{subfig:paths}-bottom.

%Then, for an given external force ${f_i}$, there exists a set of bimanual grasps using which the manipulators can resist the external force. For each grasp in the set, there may be multiple arm configurations. If there is at least one feasible arm configuration at that grasp points, the grasp is regraded to be feasible to resist the external force. For a given external force, there exists a region in the grasp space in which all the grasp points are feasible to resist the force. Here we call the region \textit{grasp feasibility region}. For example, given three external forces 
%$\left\{ {{f_1},{f_2},f{}_3} \right\}$, there exists regions in the grasp space as shown in Fig. \ref{subfig:graspspace} corresponding to them.

For a multi-manipulator system with redundant degrees of freedom, given a grasp in the grasp space and a pose of the object, we can find a set of manipulator configurations to realize the grasp. We define a grasp to be feasible under force ${f_i}$, if there is at least one manipulator configuration such that the grasp configuration (i.e. the grasp and manipulator joint angle configuration) is feasible under ${f_i}$ as defined in Sec.~\ref{sec:feasibility}.
Given an external force ${f_i}$, there is a set of such grasps in the grasp space. We call this set the\textit{ grasp feasibility region} for force ${f_i}$. For example, in Fig. \ref{subfig:paths}, the blue, red and green areas illustrate the grasp feasibility regions for $f_1$, $f_2$ and $f_3$ respectively.
This means for any grasp in the region, there is at least one manipulator configuration associated with it such that the combined grasp configuration is feasible.

Given a sequence of external forces $F:\left\{ {{f_1}, \ldots ,{f_N}} \right\}$, the multi-step manipulation planning problem is then to find a path that goes through the corresponding sequence of grasp feasibility regions such that we minimize the number of regrasps. If a grasp change is parallel to the vertical axis or the horizontal axis, it corresponds to changing the position of only one gripper. For example, in Fig. \ref{subfig:paths}, when the external forces change from ${f_2}$ to ${f_3}$: 1) if the planner chooses the horizontal connection from $G2$ to $G8$, only the left gripper needs to move; 2) if the planner chooses the vertical connection from $G2$ to $G6$, only the right gripper needs to move; 3) instead, if the planner chooses a connection from $G2$ to $G7$, both grippers need to move. We prefer horizontal or vertical connections.
%motion to a diagonal motion between the grasp feasibility regions.

Finding the exact continuous boundaries of the grasp feasibility regions is difficult. Therefore we use sampling to approximate these regions. Since we prefer horizontal or vertical connections, we sample the grasp space on a uniform grid as shown in Fig. \ref{subfig:samples}, giving many grasps along the same horizontal or vertical lines. After sampling, for each sample, we compute a set of inverse kinematic (IK) solutions to find a set of manipulator configurations to realize the grasp. For each of these IK solutions and the grasp, we check whether it is feasible to resist the external force $f_i$ using the method in Sec. \ref{sec:feasibility}. If there is at least one IK solution for the grasp that is able to resist $f_i$, we label the sample as a feasible grasp for $f_i$.

\subsection{Manipulation graph}

%After sampling and the corresponding feasibility checking in the grasp space, for each given external force ${f_i}$, we can get a subset ${S_i}$ of samples in which all the grasp candidates are feasible to resist it. The problem is then to choose one grasp from the set ${S_i}$ of each external force ${f_i}$ to produce a manipulation plan that minimizes the number of regrasps.  
%\input{Implementation/vj_verification/figs/fig_verification.tex}
We propose to build a directed weighted graph to facilitate the searching of appropriate manipulation plans as shown in Fig.~\ref{subfig:graph}.  In the manipulation graph, the nodes in the ${i^{th}}$ column corresponds to the grasp samples which are feasible to resist the external force ${f_i}$. Then we create a connection from a node in ${i^{th}}$ column to a node in ${(i + 1)^{th}}$ column, if there exists appropriate collision-free motions, a possible trajectory ${t_i}$,  by which the manipulators can move from the former node/configuration to the next. We associate each link with a weight using the number of gripper moves required from one node to the other. For example, the weight between the node $G2$ in the first column and the node $G2$ in the second column is zero, since the two nodes are the same grasp sample in the grasp space. Similarly, if the two nodes are on the same horizontal or vertical line, such as the node $G2$ for $f_2$ and $G8$ for $f_3$,  the weight for the link between them is one. Otherwise, the weight would be two. Note that one can come up with other weighting schemes. e.g., one that takes into account the trajectory length.


At this point,  the multi-step manipulation planning problem can be formulated as graph search. We want a path that starts from one node in the leftmost column for ${f_1}$ and ends with a node in the rightmost column for ${f_N}$.
We can search the manipulation graph for an optimal path. Here we use \textit{Dijkstra's algorithm} to search the graph and it gives us the manipulation plan with the least number of gripper moves based on the current set of samples.
We call this planner the \textit{min-regrasp} planner. 

Building the manipulation graph requires knowing the sequence of external forces $F$ beforehand. If the forces are revealed one by one, then the graph can be formed as the next force is specified, and it can be searched greedily. We call this version the \textit{greedy planner}.

The basic algorithm above requires a collision-free motion trajectory to be planned
between every pair of nodes in consecutive columns of the graph.
This can place a heavy burden on the planning time, because
each such motion plan is computationally expensive.
%Running a planner between every pair of nodes can place a heavy burden on the planning time.
However, in settings where a motion trajectory is likely to be found
between two grasp configurations, a \textit{lazy planning}
\cite{bohlin2000path,hauser2015lazy} approach can be taken. It
assumes valid links between nodes and delays the motion planning to be performed after the graph-search,
so that motion trajectories are planned only
between consecutive nodes in the solution sequence. If a motion trajectory cannot be
found between two nodes, the link between those nodes can be removed and
graph-search can be repeated. In our experiments, our robot was almost always
able to find motion plans between different grasp configurations. Therefore
we used this lazy version of the planners.





==> Regrasp/Regrasp.tex <==
\section{bimanual Regrasp planning without placements}
\label{sec:regrasp} 

%\input{Regrasp/fig/regraspgraph}

In this section, we introduce the definitions required to describe the problem of bimanual regrasp from $g_s$ to $g_t$ without placements and propose a multi-step planning framework. In this framework, a set of intermediate feasible bimanual and unimanual grasp configurations are identified as alternatives to object placements for regrasp planning.

\subsection{Problem representation}

\begin{figure*}[thbp]
	\begin{center}
		\subfigure[]{{
				\label{subfig:structure}
				\includegraphics[width=3.2in, angle=-0]{Regrasp/fig/integrated}}}	
		\subfigure[]{{
				\label{subfig:pose}
				\includegraphics[width=3.2in, angle=-0]{Regrasp/fig/integrated2}}}	
                \caption{Three-level planning: A solution is a path going through an alternate sequence of bimanual and unimanual grasp manifolds connected by configurations in their intersections. Each intermediate configuration in level two is a composite configuration $\left(q_{l},q_{r},T_{o}\right)$ at which the robot can release off or regrasp the object as show in Fig.~\ref{subfig:pose} . For simplicity, we did not draw robot arms in the Fig.~\ref{subfig:structure}.}
		\label{fig:structure}
	\end{center}
	\vspace{-5mm}
\end{figure*}

Consider a 3D workspace with a robot and a movable object $O$ in the environment $\varepsilon$. The robot has two manipulators,  each equipped with a parallel jaw gripper. The rigid object $O$ can only move when grasped by one or both grippers.

Let $C{S_l}$, $C{S_r}$ be the configuration space of the left and right manipulator and $C{S_o}$ the configuration space of the manipulated object. The composite configuration space $CS$ of the system is their Cartesian product $CS = C{S_l} \times C{S_r} \times C{S_o}$. Each composite configuration $q$ in $CS$ can then be written as $q = \left( {{q_l},{q_r},T} \right)$, where ${q_l} \in C{S_l}$, ${q_r} \in C{S_r}$ and $T \in C{S_o}$.

Let $g_{l}$ and $g_{r}$ be the \textit{grasp} on the object by the left and right gripper repectively. If not otherwise specified, in this section we refer to a grasp as a bimnual grasp $g=\left(g_{l},g_{r}\right)$.  A grasp $g$ represents an unimanual grasp if  $g_{l}=\varnothing$ or $g_{r}=\varnothing$. Note that given the object pose $T$, there can be more than one composite configuration $q=\left( {{q_l},{q_r},T} \right)$ corresponding to the same grasp configuration $\left( {{g_l},{g_r},T} \right)$ due to the redundancy of manipulators.
For convenience, we define a function $g\leftarrow MapConfigToGrasp\left(q\right)$, which projects a composite configuration $q$ to its grasp $g$.

The domains in $CS$ where the object $O$ is grasped by only the left and right manipulator are denoted as $C{G_l}$, $C{G_r}$ respectively, while the domain in $CS$ where the object $O$ is grasped by both manipulators is denoted as $C{G_b}$.  They are all subdimensional manifolds in $CS$ with a foliation structure induced by different grasps. Each foliation $M$ is parameterized by its grasp $g$. 

%As shown in Fig.~\ref{fig:cs}, 
The configuration space $CS$ for a bimanual regrasp planning problem consists of a collection of infinite bimanual and unimannual grasp manifolds. In theory, the planner can explore as many grasp manifolds as possible to find a solution from $q_{s}$ to $q_{t}$. A solution to the regrasp planning from $q_{s}$ to $q_{t}$ consists of a sequence of \textit{tranfer }paths connected by\textit{ release} and \textit{regrasp} operations. In the solution, moving within one grasp manifold corresponds to a transfer path, while moving between different grasp manifolds corresponds to release or regrasp operations.

In this context, the problem is reduced to picking up a finite sequence of grasp manifolds  $\left\{M\left(g_{i}\right)\right\}\left(i=1,2,...,n\right)$ in $CS$ and exploring their connectivity to find manipulation trajectories $T$ for regrasping. 

\begin{figure*}[bthp]
	\begin{center}
		\subfigure[A regrasp graph from $g_1$ to $g_2$.]{{
				\label{subfig:regraspsolution}
				\includegraphics[width=3.1 in, angle=-0]{Regrasp/fig/solution.pdf}}}
		\subfigure[$g_{s}\rightarrow g_{t}.$]{{
				\label{subfig:prob}
				\includegraphics[width=3. in, angle=-0]{Regrasp/fig/path2}}}
		
		\caption{The planner can explore the regrasp graph to find possible candidate \textit{regrasp paths} from  $g_{s}$ to  $g_{t}$.}
		\label{fig:regraspsolution}
	\end{center}
	\vspace{-5mm}
\end{figure*}

\subsection{Multi-step regrasp planning}

 In this section, we represent the connectivity in three levels: grasps, grasp manifolds, and intersections among manifolds. Fig.~\ref{fig:structure} shows the top-level structure of our regrasp planner,with detailed procedure given in Alg.~\ref{alg:alg1}:
\begin{itemize}
	\item Check the connectivity of grasps: construct a \textit{regrasp graph} $RG$ which consists of the start and target grasp $g_s$, $g_t$, and a group of intermediate bimanual and unimanual grasps $G_{candidate}$.
	\item Check the connectivity of grasp manifolds: for every two neighboring grasp manifolds $M_{i}$, $M_{j}$, sample a set of feasibe configurations in their intersection $M_{i}\cap M_{j}$ to represent their connectivity.
	\item Check the connectivity of intersections among manifolds: closed-chain and single-arm motion planners are applied to check the connectivity of sampled configurations in intersections.
\end{itemize}

%A bimanual regrasp without placements can be decomposed into an alternate sequence of finite dual-arm and single-arm motions, which are conneted by release and \underline{re-place} operations. Ideally, the robot can regrasp by directly releasing and re-placing the involved grippers on the object without transfering the manipulated object to intermediate configurations, such as regrasping a light object. However, in most cases, such as manipulating heavy or large objects, a bimamual regrasp may induce multiple intermediate grasp adjustments and object reorientations.

\subsubsection{Conectivity of Grasps}

Our planner starts by generating a set of candidate grasps $G_{candidate}$, which serve as alternatives to the object placements generally used for regrasp planning. %Both existing strategies and new methods can be applied to generate such a set of intermediate grasps. 
In this paper, we generate these grasps by sampling from the grasp space a finite number of candidate grasps and sample more if no solution from $g_{s}$ to $g_{t}$  is found.


Fig.~\ref{fig:regraspsolution} represents the connectivity of these grasps as a \textit{regrasp graph} $RG$. Each node in the graph is a bimanual or unimanual grasp. A pair of grasps is connected by a link if they share a common unimanual grasp on the object. Then, the planner can explore the graph to find possible candidate \textit{regrasp paths} from  $g_{s}$ to  $g_{t}$. Fig.~\ref{subfig:prob} illustrates the two shortest grasp solutions. 
A candidate regrasp path $G$ consists of an sequence of connected bimanual and unimanual grasps $\left\{g_{i}\right\}\left(i=1,2,...,n\right)$ including $g_s$ and $g_t$. It acts as an abstract plan to guide the search of regrasp solutions, and contracts the planning into a concrete and finite group of grasp manifolds $\left\{M\left(g_{i}\right)\right\} \left(i=1,2,...,n\right)$. 

\subsubsection{Connectivity of Grasp Manifolds}

A regrasp path provides necessary but not sufficient conditions of the connectivity of their corresponding grasp manifolds $\left\{M\left(g_{i}\right)\right\} \left(i=1,2,...,n\right)$. As shown in Fig.~\ref{fig:structure}, two neighboring grasp manifolds are connected if they intersect in $CS$ with a set of configurations at which one gripper can release off or regrasp the object. Meanwhile, every two neighboring intersections are connected by dual-arm or single-arm motions within grasp manifolds. Then, the bimanual regrasp planning is reduced to identify the structure of the intersections among neighboring grasp manifolds (i.e., check their connectivity ) and then explore the connectivity  of these intersections. 

Sample-based planners can be applied to capture the structure of the intersection $M\left(g_{i}\right)\cap M\left(g_{i+1}\right)$  between two neighboring grasp manifolds. %For example, we can build a subroadmap for each intersection \cite{simeon2004manipulation} and connect these subroadmaps to generate a manipulation solution. 
In this paper, given two grasp manifolds, instead of exploring the complete structure of their intersection, our planner simply samples a set of feasible object poses along with one of their IK solutions $I : \left\{\left(q_{l},q_{r},T_{o}\right)_{j}\right\} \left( j=1,2,...,m \right) $ as representatives for the intersection, since we focus on quickly finding one possible solutions. %\textit{The set size $M$ depends on the difficulty of find feasible configurations in the grasp manifolds.}
Each composite configuration $q^{'}$ in the sample set acts as a candidate \textit{point connection} in the final solution path, while the path segments represent bimanual or unimanual transfer paths that can be checked by closed-chain or single-arm motion planners.

\subsubsection{Connectivity of Manifold Intersections}
To generate continuous regrasp motions, i.e., check the connectivity of the intersections  among grasp manifolds, our planner uses depth-first search to find connected trajectory from $q_{s}$ to $q_{t}$ as shown from line 2 to line 20 in function $ExploreRegraspGraph$. It recursively extends a path from $q_s$ to an intermediate configuration in the subsequent intersection using a bimanual or unimanual transfer path until it reaches the target configuration $q_{t}$. 
Extending a path to an intermediate configuration is equivalent to connecting every two configurations in the same grasp manifold. It induces a pose-constrained manipulation planning problem that can be solved by existing sampled-based planners, such as CBiRRT \cite{berenson2011task}.

 \input{Regrasp/algorithm1}




==> Regrasp/algorithm1.tex <==
\begin{algorithm}[hp]
%\ContinuedFloat
\caption{Regrasp planner} 
\label{alg:alg1}
\hspace*{0.0in} {\bf} 
$RGPlanner\left(q_{s},q_{t},O\right)$:
\begin{algorithmic}[1]
\State $g_{s}, g_{t}\leftarrow MapConfigToGrasp\left(q_{s}, q_{t}\right)$
\State $T=\left\{\right\},Num\leftarrow 1$	
\While{time is not exhausted} 
	\State $G_{candidate}\leftarrow SampleGraspSpace(Num+\triangle)$
	\State $RG\leftarrow  ConstructReraspGraph\left(g_{s},g_{t}, G_{candidate}\right)$
　　	\State $T=ExploreRegraspGraph\left(q_{s},q_{s},g_{s},g_{t},RG\right)$
　　	\If {$T$ is nonempty}
	\State　		\Return $T$
　　	\EndIf
\EndWhile
\State \Return $T$
\end{algorithmic}

\vspace{0.05in}
\hspace*{0.0in} {\bf} 
$ExploreRegraspGraph\left(q_{s},q_{s},g_{s},g_{t},RG\right):$
\begin{algorithmic}[1]
	\State $G\leftarrow\left\{\right\}$,  $G^{'} \leftarrow\left\{g_{s}\right\}$, $Q\leftarrow\left\{\right\}$, $Q^{'}\leftarrow\left\{q_{s}\right\}$, $T=\left\{\right\}$
	\While{ $G^{'}$ is nonempty} 
	\State $g\leftarrow UnstackAGrasp\left(G^{'}\right)$
	\State $q\leftarrow UnstackAConfig\left(Q^{'}\right)$
	\If{$g==g_{t}$} 
	\State   Stack $g_{t}$ in $G$, $q_{t}$ in $Q$
	\State  $T \leftarrow GenerateTrajectory\left(q_{s},q_{t},Q\right)$ 
	\State \Return $T$
	\Else 
		\For{each unexplored $g^{'}$ adjacent to $g$ in $RG$} 
				\State $I\leftarrow SampleIntersection\left(g,g^{'}\right)$
				\State $connect,q^{'}\leftarrow ConnectToIntersection\left(g,q,I\right)$
				\If{$connect$}
					\State Stack $g^{'}$ in $G^{'}$, $q^{'}$ in $Q^{'}$, $g$ in $G$, $q$ in $Q$
					\State Break
					
				\Else
					\If{$g^{'}$ is the last grasp adjacent to $g$}
					\State $G^{'} \leftarrow\left\{ UnstackAConfig\left(G\right)\right\}$
					\State $Q^{'} \leftarrow\left\{ UnstackAConfig\left(Q\right)\right\}$
					\EndIf					
				\EndIf															
		\EndFor
	

	\EndIf
	\EndWhile
	
\State \Return $T$
\end{algorithmic}

\vspace{0.05in}
\hspace*{0.0in} {\bf}  
$SampleIntersection\left(g,g^{'}\right):$
\begin{algorithmic}[1]
\State $I\leftarrow \left\{\right\}, i\leftarrow0$
\While{$i <  m$} 
\State Sample $q= \left(q_{l},q_{r},T_{o}\right)$ in $CS$
\If {  the configuration $q$ is feasible for both $g$, $g^{'} $}
\State Add $q$ in $I$
\State $i\leftarrow {i+1}$
\EndIf

\EndWhile
\State \Return $I$
\end{algorithmic}

\vspace{0.05in}
\hspace*{0.0in} {\bf} 
$ConnectToIntersection\left(g,q,I\right):$
\begin{algorithmic}[1]
	\State $Success \leftarrow False, q^{'} =\left[ \right]$
	\For {each configuration $q^{'}$ in $I$}
	\If {$g$ is a bimanual grasp}
	\State	$T \leftarrow PlanClosedChainMotion\left(q,q^{'}\right)$
	\Else 
	\State $T  \leftarrow PlanSingleArmMotion\left(q,q^{'}\right)$
	\EndIf
	
	\If {$T$ is nonempty}
	\State	\Return $True, q^{'}$
	
	\Else
	
	\If {$q^{'}$ is the last item}
	\State	\Return $Success, q^{'}$
	\EndIf
	
	
	\EndIf
			
	\EndFor
	\State \Return $Success, q^{'}$
\end{algorithmic}
\end{algorithm}



==> problemDefinition/fig/document.tex <==
\begin{figure}[tp]
	\begin{center}
		\mbox{
			\subfigure[Task: Four drills \& one cut]{{
					\label{fig:cutting:a}  
					\includegraphics[width=1.6in, angle=-0]{problemDefinition/fig/task}}}

			\subfigure[Drill1 - Grasp1]{{
					\label{fig:cutting:b}  
					\includegraphics[width=1.6 in, angle=-0]{problemDefinition/fig/cutting-1}}}
		}

		\mbox{
			
			
			\subfigure[Drill2 - Grasp1]{{
					\label{fig:cutting:c}  
					\includegraphics[width=1.6 in, angle=-0]{problemDefinition/fig/cutting-2}}}
									
			\subfigure[Drill3 - Grasp2 (regrasp)]{{
					\label{fig:cutting:d}  
					\includegraphics[width=1.6 in, angle=-0]{problemDefinition/fig/cutting-3}}}

		}




		\mbox{


			
			\subfigure[Drill4 - Grasp2]{{
					\label{fig:cutting:e}  
					\includegraphics[width=1.6 in, angle=-0]{problemDefinition/fig/cutting-4}}}			
			
			\subfigure[Cutting - Grasp 3 (regrasp)]{{
					\label{fig:cutting:f}  
					\includegraphics[width=1.6 in, angle=-0]{problemDefinition/fig/cutting-6}}}			
		}

	
		\caption{Drilling\&cutting task. }
		\label{fig:cutting}
	\end{center}
\end{figure}

==> problemDefinition/fig/regraspgraph.tex <==
\begin{figure*}[tp]
	\begin{center}
		\mbox{
			
			\subfigure[A candidate regrasp Graph]{{
					\label{subfig:regraspgraph}
					\includegraphics[width=2.5 in, angle=-0]{Regrasp/fig/regraspgraph.pdf}}}
			
			\subfigure[Twp shortest grasp solution to regrasp from $g_1$ to $g_2$]{{
					\label{subfig:regraspsolution}
					\includegraphics[width=2.5 in, angle=-0]{Regrasp/fig/solution.pdf}}}	
			
		}	
		\caption{Regrasp graph and two grasp solutions.}
		\label{fig:solution}
	\end{center}
\end{figure*}
